First Run II Measurement of the W Boson Mass

We describe a measurement of the W boson mass mW using 200/pb of root-s = 1.96 TeV p-pbar collision data taken with the CDF II detector. With a sample of 63,964 W -> e nu candidates and 51,128 W -> mu nu candidates, we measure mW = [80.413 +- 0.034 (stat) +- 0.034 (sys) = 80.413 +- 0.048] GeV/c^2. This is the single most precise mW measurement to date. When combined with other measured electroweak parameters, this result further constrains the properties of unobserved particles coupling to W and Z bosons.

==> nonlinearity.tex <==
The light deposited at the front end of the electromagnetic 
calorimeter travels a larger distance through the light 
guide to the phototube, and loses a larger fraction of the 
initial light due to attenuation than the light deposited 
at the back.  This causes a lower response on average in 
the front end of the calorimeter than in the back end.  
Higher energy particles deposit a higher fraction of 
energy in the back end of the calorimeter, resulting in a 
higher response for high energy particles than for low 
energy particles.  
\par
Since photons do not lose energy due to ionization, they
typically shower deeper than electrons.  Using a model
of linearly increasing response with calorimeter depth,
we find that the integrated depth response $\Delta R_{EM}(E_T)$
corresponds to a ($0.40 \pm 0.25$)\% higher overall response 
to photons than to electrons.  We include this correction in 
our calorimeter response model.
\par

